BlockIoT: Blockchain-based Health Data Integration using IoT Devices

The development and adoption of Electronic Health Records (EHR) and health monitoring Internet of Things (IoT) Devices have enabled digitization of patient records and has also substantially transformed the healthcare delivery system in aspects such as remote patient monitoring, healthcare decision making, and medical research. However, data tends to be fragmented among health infrastructures and prevents interoperability of medical data at the point of care. In order to address this gap, we introduce BlockIoT that uses blockchain technology to transfer previously inaccessible and centralized data from medical devices to EHR systems, which provides greater insight to providers who can, in turn, provide better outcomes for patients. This notion of interoperability of medical device data is possible through an Application Programming Interface (API), which serves as a versatile endpoint for all incoming medical device data, a distributed file system that ensures data resilience, and knowledge templates that analyze, identify, and represent medical device data to providers. Our participatory design survey on BlockIoT demonstrates that BlockIoT is a suitable system to supplement physicians' clinical practice and increases efficiency in most healthcare specialties, including cardiology, pulmonology, endocrinology, and primary care.

==> README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de

